How Does Counterfactually Augmented Data Impact Models for Social Computing Constructs?

As NLP models are increasingly deployed in socially situated settings such as online abusive content detection, it is crucial to ensure that these models are robust. One way of improving model robustness is to generate counterfactually augmented data (CAD) for training models that can better learn to distinguish between core features and data artifacts. While models trained on this type of data have shown promising out-of-domain generalizability, it is still unclear what the sources of such improvements are. We investigate the benefits of CAD for social NLP models by focusing on three social computing constructs -- sentiment, sexism, and hate speech. Assessing the performance of models trained with and without CAD across different types of datasets, we find that while models trained on CAD show lower in-domain performance, they generalize better out-of-domain. We unpack this apparent discrepancy using machine explanations and find that CAD reduces model reliance on spurious features. Leveraging a novel typology of CAD to analyze their relationship with model performance, we find that CAD which acts on the construct directly or a diverse set of CAD leads to higher performance.

==> counterfactual data and explanations/ethics.tex <==
\section{Ethical Considerations}
% see: 

In this work, we attempt to understand the connection between training on counterfactually augmented data and increased model robustness. Our work centers on social NLP constructs like sexism and hate speech, whose manifestations in data can be harmful and potentially traumatizing to researchers. Furthermore, the sensitive nature of this data has the potential of victimising or re-victimizing the people referred to in them. Therefore, in accordance with ethical guidelines~\cite{vitak2016beyond,zimmer2017internet,vidgen2020directions} we conduct our analyses on aggregate data only and do not infer any attributes of the speakers in the data. We release a dataset which only contains the IDs of the original data and the typology labels we annotate.

Following common practice in NLP, we use a gendered lexicon that only contains gendered words based on the gender binary. We acknowledge that this practice is exclusionary towards non-binary individuals. We alleviate this to a certain extent by having a broader and more detailed list of identity terms, which also contains hateful terms and slurs directed towards non-binary people. In future, we hope to adopt a more intersectional perspective which is more inclusive of the sexism faced by trans and non-binary people~\cite{serano2016whipping,winter2009transpeople}. 

Constructs like sexism and hate speech detection are often depicted as neutral or objective but they are deeply contextual, subjective and ambiguous~\cite{vidgen2019challenges,jurgens2019just,nakov2021detecting}, where misclassifications can cause harm~\cite{blackwell2017classification}. We use lexica to determine core features of sexism or hate speech, but we acknowledge that both of these may manifest in context-dependent ways and there is no single objective determinant of hate speech or sexism (or even sentiment). Furthermore, promoting features like identity terms can increase the risk of misclassifying non-hate content with such terms, such as disclosure or reports of facing hate speech, leading to unintended bias~\cite{blodgett2020language}. 
%Following up on this subjectivity and based on recommendations by \citet{blodgett2020language}, we motivate our analyses of unintended bias on normative grounds, situated in the context of the harms wrought by misclassification of content containing identity terms despite being non-sexist or non-hate speech. We acknowledge that we only study one type of unintended bias and there are other aspects that require further investigation~\cite{blackwell2017classification}.  

We do not undertake any further data generation or data annotation by human subjects, as we use data made available by previous researchers and use lexica for annotating counterfactual types. Nonetheless, as we show the potential of CAD in improving some aspects of model robustness, we hope that the community will adopt annotation guidelines that factor in the risk of harm that annotators and CAD designers working on abusive language might face~\cite{vidgen2020directions}. 

We aim to understand how CAD improves model robustness, but we acknowledge and caution that these types of data augmentation can also be used to poison NLP models and cause them to have several harmful properties~\cite{wallace2020customizing,sun2018data}.


==> counterfactual data and explanations/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
